Verification Challenges in Sparse Matrix Vector Multiplication in High Performance Computing: Part I

Sparse matrix vector multiplication (SpMV) is a fundamental kernel in scientific codes that rely on iterative solvers. In this first part of our work, we present both a sequential and a basic MPI parallel implementations of SpMV, aiming to provide a challenge problem for the scientific software verification community. The implementations are described in the context of the PETSc library.

==> eptcsdata.tex <==
\providecommand{\firstpage}{98}
\providecommand{\publicationstatus}{S.F.\ Siegel and G.\ Gopalakrishnan (Eds.):\\
International Workshop on Verification of\\
Scientific Software (VSS 2025)\\
EPTCS 432, 2025, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.432.11}{10.4204/EPTCS.432.11}}
\pdfoutput=1

